Proto-lm: A Prototypical Network-Based Framework for Built-in Interpretability in Large Language Models

Large Language Models (LLMs) have significantly advanced the field of Natural Language Processing (NLP), but their lack of interpretability has been a major concern. Current methods for interpreting LLMs are post hoc, applied after inference time, and have limitations such as their focus on low-level features and lack of explainability at higher level text units. In this work, we introduce proto-lm, a prototypical network-based white-box framework that allows LLMs to learn immediately interpretable embeddings during the fine-tuning stage while maintaining competitive performance. Our method's applicability and interpretability are demonstrated through experiments on a wide range of NLP tasks, and our results indicate a new possibility of creating interpretable models without sacrificing performance. This novel approach to interpretability in LLMs can pave the way for more interpretable models without the need to sacrifice performance.

==> emnlp2023-latex/sections/interpretability.tex <==


% plausibility \cite{lage2019evaluation, deyoung2019eraser, hase2019interpretable, chan2022unirex}. 

\subsection{Simulatability Evaluation}
Simulatability refers to the ability of humans to replicate the model's decision when provided with its explanations \cite{doshi2017towards}. A good interpretability method should aid humans in understanding and reproducing the model's reasoning.
In order to evaluate the interpretability of our proposed method, \texttt{proto-lm}, we employed a human-in-the-loop approach. We used Amazon Mechanical Turk to crowdsource our evaluations and presented 3 workers with 50 examples each from the SST-2 and QNLI datasets, along with explanations for the model's decisions. As a baseline, we presented the workers with randomly-selected examples from the training set as explanations. To evaluate \texttt{proto-lm}, we presented another set of 3 workers with the same examples but with explanations provided by the prototypes of \texttt{proto-lm}. Specifically, we provided the 5 closest prototypes to the input from the prototypical layer of the best-performing model on that task. 

Additionally, we also compared \texttt{proto-lm}'s simulatability against 3 other well-known interpretability methods: LIME, Integrated Gradients, and Guided Backprop. We employed three workers for each example and reported the mean percentage of examples where the workers correctly replicated the model's decision in Table \ref{tab:simul_table}. Our results indicate that \texttt{proto-lm} allows the workers to replicate the model's decisions better than all the other interpretability methods on both tasks.


==> emnlp2023-latex/tables/K_table.tex <==
\begin{table*}[!ht]
\centering
%\small
\begin{tabular}{lccccccc}
\hline
     & \textbf{$K$=1} & \textbf{$K$=10}  & \textbf{$K$=50}  &  \textbf{$K$=100} &  \textbf{$K$=250}  & \textbf{$K$=375}  & \textbf{$K$=500} \\
        \hline
        \hline
   \textbf{SST-2} &91.2 & 92.4 & 92.8 & 93.3 & \textbf{96.4} & 96.3 & 96.1 \\
        \hline
        \textbf{IMDb} & 90.1 & 90.4 & 91.2 &92.9 &\textbf{95.8} & 95.6 & 95.0 \\
        
        \hline 
\end{tabular}
  \caption{Predictive accuracy of \texttt{proto-lm} on RoBERTa-large when varying $K$, the hyperparameter for cluster size in prototypical space.}
    \label{tab:K_table}
    %\vspace{5pt}
\end{table*}

==> emnlp2023-latex/tables/performance_table.tex <==
\begin{table*}[!t]
\small
\centering
\begin{tabular}{l|c|c|c|c|c|c|c}
\multicolumn{1}{l}{\textbf{}} & \multicolumn{1}{c}{\textbf{SST-2}}  & \multicolumn{1}{c}{\textbf{QNLI}}  & \multicolumn{1}{c}{\textbf{MNLI}}  &  \multicolumn{1}{c}{\textbf{WNLI}} & \multicolumn{1}{c}{\textbf{RTE}} &  \multicolumn{1}{c}{\textbf{IMDb}}  & \multicolumn{1}{c}{\textbf{SST-5}} \\
\hline
\hline
\multicolumn{1}{l}{\text{BERT-base-uncased} \cite{devlin2018bert}} & \multicolumn{1}{c}{93.2} & \multicolumn{1}{c}{90.5} & \multicolumn{1}{c}{84.6} & \multicolumn{1}{c}{46.4$^*$} & \multicolumn{1}{c}{66.4} & \multicolumn{1}{c}{91.3} & \multicolumn{1}{c}{54.9} \\
\hdashline
\multicolumn{1}{l}{\text{BERT-base-uncased + \texttt{proto-lm}}} & \multicolumn{1}{c}{\textbf{93.6}} & \multicolumn{1}{c}{90.2} & \multicolumn{1}{c}{84.0} & \multicolumn{1}{c}{\textbf{47.9}} & \multicolumn{1}{c}{\textbf{68.1}} & \multicolumn{1}{c}{\textbf{91.5}} & \multicolumn{1}{c}{\textbf{55.3}} \\

\hline

\multicolumn{1}{l}{\text{BERT-large-uncased} \cite{devlin2018bert}} & \multicolumn{1}{c}{94.9} & \multicolumn{1}{c}{92.7} & \multicolumn{1}{c}{86.7} & \multicolumn{1}{c}{47.9$^*$} & \multicolumn{1}{c}{70.1} & \multicolumn{1}{c}{92.0} & \multicolumn{1}{c}{56.2} \\
\hdashline
\multicolumn{1}{l}{\text{BERT-large-uncased + \texttt{proto-lm}}} & \multicolumn{1}{c}{\textbf{95.2}} & \multicolumn{1}{c}{92.4} & \multicolumn{1}{c}{86.3} & \multicolumn{1}{c}{47.9} & \multicolumn{1}{c}{\textbf{76.2}} & \multicolumn{1}{c}{\textbf{93.6}} & \multicolumn{1}{c}{\textbf{56.4}} \\

\hline

\multicolumn{1}{l}{\text{RoBERTa-base} \cite{liu2019roberta}} & \multicolumn{1}{c}{93.6} & \multicolumn{1}{c}{92.5} & \multicolumn{1}{c}{87.2} & \multicolumn{1}{c}{$56.3^{*}$} & \multicolumn{1}{c}{78.7} & \multicolumn{1}{c}{94.7} & \multicolumn{1}{c}{56.4} \\
\hdashline
\multicolumn{1}{l}{\text{RoBERTa-base + \texttt{proto-lm}}} & \multicolumn{1}{c}{\textbf{94.0}} & \multicolumn{1}{c}{92.2} & \multicolumn{1}{c}{86.9} & \multicolumn{1}{c}{56.3} & \multicolumn{1}{c}{\textbf{84.2}} & \multicolumn{1}{c}{\textbf{95.0}} & \multicolumn{1}{c}{\textbf{56.8}} \\

\hline

\multicolumn{1}{l}{\text{RoBERTa-large} \cite{liu2019roberta}} & \multicolumn{1}{c}{96.4} & \multicolumn{1}{c}{94.7} & \multicolumn{1}{c}{90.2} & \multicolumn{1}{c}{$56.4^{*}$} & \multicolumn{1}{c}{86.6} & \multicolumn{1}{c}{95.6} & \multicolumn{1}{c}{57.9} \\
\hdashline
\multicolumn{1}{l}{\text{RoBERTa-large + \texttt{proto-lm}}} & \multicolumn{1}{c}{\textbf{96.5}} & \multicolumn{1}{c}{94.6} & \multicolumn{1}{c}{90.1} & \multicolumn{1}{c}{56.4} & \multicolumn{1}{c}{\textbf{88.6}} & \multicolumn{1}{c}{\textbf{95.8}} & \multicolumn{1}{c}{\textbf{58.0}} \\
\hline
\multicolumn{1}{l}{\text{BART-Large} \cite{lewis2019bart}} & \multicolumn{1}{c}{96.6} & \multicolumn{1}{c}{94.9} & \multicolumn{1}{c}{90.2} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{87.0} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} \\
\hdashline
\multicolumn{1}{l}{\text{BART-Large + \texttt{proto-lm}}} & \multicolumn{1}{c}{\textbf{97.0}} & \multicolumn{1}{c}{94.2} & \multicolumn{1}{c}{89.3} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{\textbf{89.2}} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} \\


\hline
\hline


\end{tabular}

\caption{Predictive accuracy of \texttt{proto-lm} compared against fine-tuned versions of their base LLM's. We observe competitive performance on all tasks, with bolded and underlined values indicating better and equivalent performances, respectively. $^*$ indicates that the performance is a result of our experiments on that task and not reported in the original work cited. All results for \texttt{proto-lm} are results under the optimal arrangement of hyperparameters for that task, which we obtain through experimentation (see Appendix \ref{hyperparameters}).}
\label{tab:performance_table}
\end{table*}
